Hardware Impairments Aware Transceiver Design for Bidirectional Full-Duplex MIMO OFDM Systems

In this paper we address the linear precoding and decoding design problem for a bidirectional orthogonal frequencydivision multiplexing (OFDM) communication system, between two multiple-input multiple-output (MIMO) full-duplex (FD) nodes. The effects of hardware distortion as well as the channel state information error are taken into account. In the first step, we transform the available time-domain characterization of the hardware distortions for FD MIMO transceivers to the frequency domain, via a linear Fourier transformation. As a result, the explicit impact of hardware inaccuracies on the residual selfinterference (RSI) and inter-carrier leakage (ICL) is formulated in relation to the intended transmit/received signals. Afterwards, linear precoding and decoding designs are proposed to enhance the system performance following the minimum-mean-squarederror (MMSE) and sum rate maximization strategies, assuming the availability of perfect or erroneous CSI. The proposed designs are based on the application of alternating optimization over the system parameters, leading to a necessary convergence. Numerical results indicate that the application of a distortionaware design is essential for a system with a high hardware distortion, or for a system with a low thermal noise variance.

==> Contributions_Overview.tex <==
 sssssssssssssssss

==> Sections/_sec_simulations.tex <==



In this section we evaluate the behavior of the studied FD MC system via numerical simulations. In particular, we evaluate the proposed designs in Sections~\ref{sec:WMMSE} and~\ref{sec:WMMSE_CSI_Error} for various system situations, and under the impact of transceiver inaccuracy and CSI error. Communication channels $\ma{H}_{ii}^k$ follow an uncorrelated Rayleigh flat fading model with variance $\rho$. For the self-interference channel we follow the characterization reported in \cite{FD_ExperimentDrivenCharact}. In this respect we have $\ma{H}_{ij} \sim \mathcal{CN}\left( \sqrt{\frac{\rho_{\text{si}} K_R}{1+K_R}} \ma{H}_0 , \frac{\rho_{\text{si}}}{1+K_R} \ma{I}_{M_{i}} \otimes \ma{I}_{N_{j}} \right)$ where $\rho_{\text{si}}$ represents the self-interference channel strength, $\ma{H}_0$ is a deterministic term,\footnote{For simplicity, we choose $\ma{H}_0$ as a matrix of all-$1$ elements.} and $K_R$ is the Rician coefficient. For each channel realization, the resulting performance is evaluated by employing different design strategies and for various system parameters. The overall system performance is then averaged over $100$ channel realizations. Unless otherwise is stated, the following values are used to define our default setup: $K = 4$, $K_R = 10$, $M:=M_i=N_j=2$, $\rho = -20~\text{dB}$, $\rho_{\text{si}} = 1$, $\sigma_{\text{n}}^2 := \sigma_{i,k}^2 = -30~\text{dB}$, $P_{\text{max}}:=P_i = 1$, $d_i=1$, $\kappa = -30~\text{dB}$ where $\ma{\Theta}_{\text{rx},i}^k = \kappa \ma{I}_{M_{i}}$ and $\ma{\Theta}_{\text{tx},i}^k = \kappa \ma{I}_{N_{i}}$, and $\zeta_{ij}^k= -15~\text{dB}$, $\forall i,j \in \mathbb{I}, \; k \in \mathbb{F}_K$. \par 

\subsection{Algorithm analysis}  \label{sec_AlgorithmAnalysis}


\begin{figure}[!t] 
    \begin{center}
        \includegraphics[angle=0,width=\MainFigureSizes]{./Figures/rand_init5.pdf}
				        %\fbox{model_rect6.pdf}
    \caption{Average convergence behavior for AltQCP and AltSDP algorithms. AltQCP converges with fewer steps, and leads to a smaller optimality gap compared to AltSDP. Both algorithms converge in $10$-$30$ iterations.} \vspace{-5mm}  \label{fig:init}
    \end{center} \vspace{-1mm} 
\end{figure}
\begin{figure}[t]  
%\hspace{0.0cm} \subfigure[Convergence]{\includegraphics[angle = 0, width = 0.66\columnwidth]{./Figures/rand_init}} \label{fig_conv1}
\subfigure[CPU Time vs $M$]{\includegraphics[width = 0.48\columnwidth]{./Figures/CC_M}} \label{fig_conv2}
\subfigure[CPU Time vs $K$]{\includegraphics[width = 0.48\columnwidth]{./Figures/CC_K}} \label{fig_conv3}
%\subfigure[CPU]{\includegraphics[width = 0.49\columnwidth]{./Figures/power}} \label{fig_conv4}
%\LoadClass[onecolumn]{article}
%\addtolength{\linewidth}{3.6in}
\caption{Comparison of the algorithm computational complexities, in terms of the required CPU time (CT), for different system dimensions.}  \vspace{-5mm}
\label{fig:Complexity}
\vspace{-4pt}
\end{figure} 

%\subsection{Algorithm analysis}  
%\begin{figure}[!t] 
    %\begin{center}
        %\includegraphics[angle=0,width=\MainFigureSizes]{./Figures/CC_M.pdf}
				        %%\fbox{model_rect6.pdf}
    %\caption{} \label{fig:Complexity_M}
    %\end{center} \vspace{-0mm} 
%\end{figure} 
%
%\subsection{Algorithm analysis}  
%\begin{figure}[!t] 
    %\begin{center}
        %\includegraphics[angle=0,width=\MainFigureSizes]{./Figures/CC_K.pdf}
				        %%\fbox{model_rect6.pdf}
    %\caption{} \label{fig:Complexity_K}
    %\end{center} \vspace{-0mm} 
%\end{figure} 

Due to the alternating structure, the convergence behavior of the proposed algorithms is of interest, both as a verification for algorithm operation as well as an indication of the algorithm efficiency in terms of the required computational effort. In this part, the performance of AltQCP and AltSDP algorithms are studied in terms of the average convergence behavior and computational complexity. Moreover, the impact of the choice of the algorithm initialization is evaluated. \\
In Fig.~\ref{fig:init} the average convergence behavior is depicted for different values of $\kappa$~[dB]. In particular, "Min" and "Avg" curves respectively represent the minimum, and the average value of the algorithm objective at the corresponding optimization step over the choice of $20$ random initializations. Moreover, "RSM" represents the right-singular matrix initialization proposed in \cite[Appendix~A]{5585631}. It is observed that the algorithms converge, within $10-30$ optimization iterations, specially as $\kappa$ is small. Although the global optimality of the final solution can not be verified due to the possibility of local solutions, the numerical experiments suggest that the applied RSM initialization shows a better convergence behavior compared to a random initialization. Moreover, it is observed that a higher transceiver inaccuracy results in a slower convergence and a gap with optimality. This is expected, as larger $\kappa$ leads to a more complex problem structure. Note that the algorithm AltQCP shows a smaller value of objective compared to that of AltSDP for any value of $\kappa$, since the impact of CSI error is not considered in the algorithm objective.   

%In Fig.~\ref{fig:Convergence_AltQCP} the average convergence behavior of the AltQCP algorithm is observed, following a similar structure as in Fig.~\ref{fig:Convergence_AltSDP}. Similar to Fig.~\ref{fig:Convergence_AltSDP}, it is observed that algorithm initialization based on RSM shows a better convergence compared to a random initialization case. 
 
In addition to the algorithm convergence behavior, the required computational complexity is affected by the problem dimension, and the required per-iteration complexity, see Subsection~\ref{alg_complexity}. In Fig.~\ref{fig:Complexity}, the required computation time (CT) is depicted for different number of antennas, as well as different number of subcarriers\footnote{The reported CT is obtained using an Intel Core i$5-3320$M processor with the clock rate of $2.6$ GHz and $8$ GB of random-access memory (RAM). As software platform we have used MATLAB $2013$a, on a $64$-bit operating system.}. It is observed that the AltSDP results in a significantly higher CT, compared to AltQCP. This is expected as the consideration of CSI error in AltSDP results in a larger problem dimension, and hence higher complexity. Moreover, the obtained closed-form solution expressions in AltQCP result in a more efficient implementation. Nevertheless, the required CT for AltQCP is still higher than the threshold-based low-complexity approaches, see Subsection~\ref{Sim_benchmarks}, due to the expanded problem dimension associated with the impact of residual self-interference and inter-carrier leakage.    

\subsection{Performance comparison}
In this part we evaluate the performance of the proposed AltSDP and AltQCP algorithms in terms of the resulting worst-case MSE, see Subsection~\ref{WC_CSI}, under various system conditions.  

\subsubsection{Comparison benchmarks} \label{Sim_benchmarks}
In order to facilitate a meaningful comparison, we consider popular approaches for the design of FD single-carrier bidirectional systems, or the available designs for other MC systems with simplified assumptions, see Subsection~\ref{related_works}. The following approaches are hence implemented as our evaluation framework:    
\begin{itemize}
\item \textit{AltSDP}:~The AltSDP algorithm proposed in Section~\ref{sec:WMMSE_CSI_Error}. The impact of the hardware distortions leading to inter-carrier leakage, as well as CSI error are taken into account.
\item \textit{AltQCP}:~The AltQCP algorithm proposed in Section~\ref{sec:WMMSE}. The algorithm operates on the simplified assumption that the CSI error does not exist, i.e., $\zeta=0$, and hence focuses on the impact of hardware distortions.   
\item \textit{HD}:~The AltSDP algorithm is used on an equivalent HD setup, where the communication directions are separated via a time division duplexing (TDD) scheme. 
%The equivalent number of data streams to the FD case is transmitted, and evaluated in terms of the resulting worst-case MSE.    
\item \textit{$\kappa=0$}:~The impact of CSI error is taken into account similar to, e.g., \cite{ZTH:132, ng2012dynamic}. Nevertheless the impact of hardware distortion, leading to inter-carrier leakage, is ignored.     
\item \textit{SC}:~The optimal single carrier design applied to the defined MC system, following a similar approach as in \cite{DMBS:12, CRYL:15}. The impact of CSI error and hardware distortions are taken into account.   
\end{itemize}
Other than the approaches that directly deal with the impact of residual self-interference, e.g., \cite{DMBS:12, CRYL:15}, a low complexity design framework is proposed in \cite{ Huberman2014, JTLH:12}, by introducing an interference power threshold, denoted as $P_{\text{th}}$. In this approach, it is assumed that the self-interference signal can be perfectly subtracted, given the self-interference power is kept below $P_{\text{th}}$. In this regard, we evaluate the extended version of \cite{JTLH:12} on the defined MC setup for three values of $P_{\text{th}}$: 
\begin{itemize}
\item \textit{$P_{\text{th}}-\{\infty, \text{High}, \text{Low}\}$}:~representing a design by respectively choosing $P_{\text{th}}=$ $\infty$, $P_i$, $P_i/10$, representing a system with perfect, high, and low dynamic range conditions. 
%This case corresponds to a linear precoder/decoder design with no consideration on the impact of self-interference. 
%\item \textit{$P_{\text{th}}-\text{High}$}:~similar to the previous case, but setting $P_{\text{th}} = P_i$. This represents a system with a relatively high dynamic range, i.e., a high tolerable self-interference power. A perfect hardware and CSI is assumed.    
%\item \textit{$P_{\text{th}}-\text{Low}$}:~similar to the previous case, but setting $P_{\text{th}} = P_i/10$. This represents a system with a relatively low dynamic range, i.e., a small tolerable self-interference power. A perfect hardware and CSI is assumed.    
\end{itemize}

\subsubsection{Visualization}

\begin{figure*}[t]  
\hspace{0.0cm} \subfigure[WC MSE vs. transceiver inaccuracy ($\kappa$)]{\includegraphics[angle = 0, width = 0.666\columnwidth]{./Figures/kappa.pdf}}
\subfigure[WC MSE vs. feasible CSI error radius ($\zeta$)]{\includegraphics[width = 0.666\columnwidth]{./Figures/zeta.pdf}} 
\subfigure[WC MSE vs. thermal noise variance ($\sigma_{\text{n}}^2$)]{\includegraphics[width = 0.666\columnwidth]{./Figures/noise.pdf}} 
%\LoadClass[onecolumn]{article}
%\addtolength{\linewidth}{3.6in}
\caption{Worst-case (WC) MSE for different system conditions. The gain of a distortion-aware design is apparent for a high SNR, or a high distortion region.}  \vspace{-3mm} 
\label{fig:WC_MSE}
\vspace{-7pt}
\end{figure*}


%\begin{figure}[!t] 
    %\begin{center}
        %\includegraphics[angle=0, width=\MainFigureSizes]{./Figures/kappa.pdf}
				        %%\fbox{model_rect6.pdf}
    %\caption{WC MSE vs. transceiver inaccuracy ($\kappa$). As transceiver accuracy degrades, the resulting MSE increases.} \label{fig:kappa}
    %\end{center} \vspace{-0mm} 
%\end{figure} 
%
%\begin{figure}[!t] 
    %\begin{center}
        %\includegraphics[angle=0, width=\MainFigureSizes]{./Figures/zeta.pdf}
				        %%\fbox{model_rect6.pdf}
    %\caption{WC MSE vs. feasible CSI error radius ($\zeta$). The resulting MSE increases as CSI accuracy degrades.} \label{fig:zeta}
    %\end{center} \vspace{-0mm} 
%\end{figure} 
%
%\begin{figure}[!t] 
    %\begin{center}
        %\includegraphics[angle=0, width=\MainFigureSizes]{./Figures/noise.pdf}
				        %%\fbox{model_rect6.pdf}
    %\caption{WC MSE vs. thermal noise variance ($\sigma_{\text{n}}^2$). Low noise regime results in a low MSE for the proposed algorithms, but degrades the performance of the algorithms with perfect hardware assumption.} \label{fig:noise}
    %\end{center} \vspace{-0mm} 
%\end{figure} 





%%%%%%%%%\begin{figure}[!t] 
    %%%%%%%%%\begin{center}
        %%%%%%%%%\includegraphics[angle=0,width=\MainFigureSizes]{./Figures/rho_h.pdf}
				        %%%%%%%%%%\fbox{model_rect6.pdf}
    %%%%%%%%%\caption{WC MSE vs. communication channel strength ($\rho$). The resulting MSE decreases as the channel strength increases, but saturates due to the impact of hardware distortion.} \label{fig:rho}
    %%%%%%%%%\end{center} \vspace{-0mm} 
%%%%%%%%%\end{figure}
 %%%%%%%%%
%%%%%%%%%\begin{figure}[!t] 
%%%%%%%%%\begin{center}
        %%%%%%%%%\includegraphics[angle=0,width=\MainFigureSizes]{./Figures/M.pdf}
				        %%%%%%%%%%\fbox{model_rect6.pdf}
    %%%%%%%%%\caption{WC MSE vs. number of antennas ($M$). The resulting MSE decreases as the number of antennas increase.} \label{fig:M}
    %%%%%%%%%\end{center} \vspace{-0mm} 
%%%%%%%%%\end{figure} 
%%%%%%%%%\begin{figure}[!t] 
%%%%%%%%%\begin{center}
        %%%%%%%%%\includegraphics[angle=0,width=\MainFigureSizes]{./Figures/K.pdf}
				        %%%%%%%%%%\fbox{model_rect6.pdf}
    %%%%%%%%%\caption{WC MSE vs. number of independent subcarriers ($K$). The resulting MSE increases as $K$ increases. The performance of SC scheme is optimal for small $K$, but degrades rapidly as $K$ increases.} \label{fig:K}
    %%%%%%%%%\end{center} \vspace{-0mm} 
%%%%%%%%%\end{figure}

%%%%%%%%%%%%%%%%%

%\begin{figure}[!t] 
%\begin{center}
        %\includegraphics[angle=0,width=\MainFigureSizes]{./Figures/kappa_sr.pdf}
				        %%\fbox{model_rect6.pdf}
    %\caption{System sum rate vs. transceiver inaccuracy ($\kappa$). As transceiver accuracy degrades, the resulting sum rate decreases.} \label{fig:SR_kappa}
    %\end{center} \vspace{-0mm} 
%\end{figure}
%
%\begin{figure}[!t] 
%\begin{center}
        %\includegraphics[angle=0,width=\MainFigureSizes]{./Figures/noise_sr.pdf}
				        %%\fbox{model_rect6.pdf}
    %\caption{System sum rate vs. thermal noise variance ($\sigma_{\text{n}}^2$). A higher sum rate is obtained for a lower noise level.} \label{fig:SR_N}
    %\end{center} \vspace{-0mm} 
%\end{figure}
%
%\begin{figure}[!t] 
%\begin{center}
        %\includegraphics[angle=0,width=\MainFigureSizes]{./Figures/power_sr.pdf}
				        %%\fbox{model_rect6.pdf}
    %\caption{System sum rate vs. maximum transmit power ($P_{\text{max}}$). A higher sum rate is obtained for a lower noise level.} \label{fig:SR_N}
    %\end{center} \vspace{-0mm} 
%\end{figure}

\begin{figure*}[t]  
\hspace{0.0cm} \subfigure[Sum rate vs. hardware inaccuracy ($\kappa$)]{\includegraphics[angle = 0, width = 0.666\columnwidth]{./Figures/kappa_sr}} \label{fig_sr_kappa}
\subfigure[Sum rate vs. noise variance ($\sigma_{\text{n}}^2$)]{\includegraphics[width = 0.666\columnwidth]{./Figures/noise_sr}} \label{fig_sr_noise}
\subfigure[Sum rate vs. maximum transmit power ($P_{\text{max}}$)]{\includegraphics[width = 0.666\columnwidth]{./Figures/power_sr}} \label{fig_sr_power}
%\LoadClass[onecolumn]{article}
%\addtolength{\linewidth}{3.6in}
\caption{Average sum rate for different system conditions. The gain of a distortion-aware design is apparent for a high SNR, or a high distortion region. The default parameter set is $\kappa= - 50~\text{dB}$, $\sigma_{\text{n}}^2 := \sigma_{i,k}^2 = -30~\text{dB}$, $P_{\text{max}}:=P_i = 1$. } \vspace{-3mm} 
\label{fig:sumrate}
\vspace{-7pt}
\end{figure*}


In Figs.~\ref{fig:WC_MSE} (a)-(c) the average performance of the defined benchmark algorithms in terms of the worst-case (WC) MSE are depicted. The average sum rate behavior of the system is depicted in Fig.~\ref{fig:sumrate} (a)-(c)\footnote{More extensive numerical evaluations have been conducted on the current setup, verifying the similar conclusions. However, the extended results are moved to \cite[Section~VI]{taghizadeh2017linear} due to the space limitations.}. \\ 

In Fig.~\ref{fig:WC_MSE}-(a) the impact of transceiver inaccuracy is depicted on the resulting WC-MSE. It is observed that the estimation accuracy is degraded as $\kappa$ increases. For the low-complexity algorithms, where the impact of hardware distortion is not considered, the resulting MSE goes to infinity as $\kappa$ increases. Nevertheless, the resulting MSE reaches a saturation point for the distortion-aware algorithms, i.e, AltSDP and AltQCP. This is since for the data streams affected with a large distortion intensity, the decoder matrices are set to zero which limits the resulting MSE to the magnitude of the data symbols. Moreover, the AltSDP method outperforms the other performance benchmarks for all values of $\kappa$. It is worth mentioning that the significant gain of an FD system with low $\kappa$ over the HD counterpart, disappears for a larger levels of hardware distortion where AltSDP and HD result in a close performance.    

In Fig.~\ref{fig:WC_MSE}-(b) the impact of the CSI error is depicted. It is observed that the estimation MSE increases for a larger value of $\zeta$. For the low-complexity algorithms where the impact of CSI error is not considered, the resulting MSE goes to infinity, as $\zeta$ increases. Nevertheless, the performance of the AltSDP method saturates by choosing zero decoder matrices, following a similar concept as for Fig.~\ref{fig:WC_MSE}-(a). It is observed that the performance of the AltSDP and AltQCP methods deviate as $\zeta$ increases, however, they obtain a similar performance for a small $\zeta$. Similar to Fig.~\ref{fig:WC_MSE}-(a), a significant gain is observed in comparison to the HD and SC cases, for a system with accurate CSI.  

In Fig.~\ref{fig:WC_MSE}-(c) the impact of the thermal noise variance is depicted. It is observed that the resulting performance degrades for the distortion-aware algorithms, as the noise variance increases. Nevertheless, we observe a significant performance degradation for the threshold-based algorithms, particularly $P_{\text{th}}-\text{Low}$, in the low noise regime. This is since the imposed interference power threshold tends to reduce the transmit power, which results in a larger decoder matrices in a low-noise regime. This, in turn, results in an increased impact of distortion. Nevertheless, as the noise variance increases, the algorithm chooses decoding matrices with a smaller norm in order to reduce the impact of noise. This also reduces the impact of hardware distortions. Similar to Fig.~\ref{fig:WC_MSE}-(a), the proposed AltSDP method outperforms the other comparison benchmarks. It is observed that the performance degradation caused by ignoring the CSI error in AltQCP, or by applying a simplified single carrier design, is significant particularly for a system with a small noise variance. 

%%%%%%%In Fig.~\ref{fig:rho} the impact of the communication channel strength is observed on the resulting system performance. It is observed that the MSE decreases in most parts as the communication channel becomes stronger. Nevertheless, the system performance saturates, due to the impact of hardware distortion which increase proportional to the transmit/receive power at each chain. Moreover, the performance of the methods with a perfect hardware/CSI assumption saturates at a higher MSE, due to the impact of the ignored effect. Moreover, the algorithms AltQCP and AltSDP result in an approximately similar performance for a system with a high channel strength. This is since for a high $\rho$ regime, the impact of thermal noise and CSI error become less significant. As a result the system performance is dominated by the impact of distortion which is amplified due to the higher channel strength. 
 %%%%%%%
%%%%%%%
%%%%%%%%In Fig.~\ref{fig:rho_si} the impact of the strength of the self-interference channel is depicted.
 %%%%%%%
%%%%%%%In Fig.~\ref{fig:M} the impact of the number of antennas is observed. As expected, a higher number of antennas results in an increased performance for all of the performance benchmarks. In particular, a higher number of antennas enables the system to better overcome the CSI error, for a fixed $\zeta$, and also to direct the transmit power in the desired channel and not in the self-interference path.   
%%%%%%%
%%%%%%%In Fig.~\ref{fig:K} the impact of the number of subcarriers is observed on the resulting MSE. It is observed that a higher number of subcarriers result in a higher error for all benchmark methods. This is expected as a higher number of subcarriers enables a higher number of communication streams, resulting in a lower available per-stream power. The performance of the SC design reaches optimality of a single carrier system, as expected. Nevertheless the performance of the SC scheme deviates from optimality as $K$ increases, and results in the highest MSE in comparison to the evaluated benchmarks, for $K \geq 5$. This is expected, as higher independent subcarriers represent a channel with a higher frequency selectivity which calls for a specialized MC design.   

In Fig.~\ref{fig:sumrate} the average sum rate behavior of the system depicted. In Fig.~\ref{fig:sumrate}-(a), the impact of hardware inaccuracy is depicted. It is observed that a higher $\kappa$ results in a smaller sum rate. Moreover, the obtained gains via the application of the defined MC design in comparison to the designs with frequency-flat assumption, and via the application of FD setup in comparison to HD setup, are evident for a system with accurate hardware conditions. Conversely, it is observed that a design with consideration of hardware impairments is essential as $\kappa$ increases. In Figs.~\ref{fig:sumrate}-(b) and (c), the opposite impacts of noise level, and the maximum transmit power are observed on the system sum rate. It is observed that the system sum rate increases as noise level decreases, or as the maximum transmit power increases. In both cases, the gain of AltQCP method, in comparison to
the methods which ignore the impact of hardware distortions are observed for a high SNR conditions, i.e., for a system with a high transmit power or a low noise level. 

%\begin{figure}[!t] 
%\begin{center}
        %\includegraphics[angle=0,width=\MainFigureSizes]{./Figures/power.pdf}
				        %%\fbox{model_rect6.pdf}
    %\caption{} \label{fig:K}
    %\end{center} \vspace{-0mm} 
%\end{figure} 

%\subsubsection{Visualization: sum rate}
%
%\begin{figure}[!t] 
    %\begin{center}
        %\includegraphics[angle=0,width=\MainFigureSizes]{./Figures/power.pdf}
				        %%\fbox{model_rect6.pdf}
    %\caption{} \label{fig:kappa}
    %\end{center} \vspace{-0mm} 
%\end{figure} 
%
%\begin{figure}[!t] 
    %\begin{center}
        %\includegraphics[angle=0,width=\MainFigureSizes]{./Figures/power.pdf}
				        %%\fbox{model_rect6.pdf}
    %\caption{} \label{fig:noise}
    %\end{center} \vspace{-0mm} 
%\end{figure} 
%
%\begin{figure}[!t] 
    %\begin{center}
        %\includegraphics[angle=0,width=\MainFigureSizes]{./Figures/power.pdf}
				        %%\fbox{model_rect6.pdf}
    %\caption{} \label{fig:power}
    %\end{center} \vspace{-0mm} 
%\end{figure} 





%
%In Fig.~\ref{fig:kappa} 
%
%In Fig.~\ref{rate_function_lowerbound} the actual value of the rate function is compared to the proposed lower bound, for different levels of CSI error intensity.
%
%\subsection{Achievable wost case performance}
%
%In Fig.~\ref{}-Fig.~\ref{} the worst-case sum rate of the system is depicted, for different values of the system parameters. In this respect, 'Scenario~$1$' represents the proposed design in Section~\ref{sec:WMMSE}. 'Scenario~$2$', 'Scenario~$3$', and 'Scenario~$4$' represent a simplified sum-rate maximizing approach, by (respectively) ignoring the impact of distortion signals, i.e., assuming $\kappa=\beta=0$, the impact of CSI inaccuracy, i.e., assuming $\zeta=0$, and jointly ignoring the impacts of chain imperfections and CSI errors. Scenario~$2$ is adopted from the proposed design in \cite{CTLMH:16}, where Scenario~$4$ is previously studied in \cite{Huberman2014, JTLH:12}. Finally, 'Scenario~$5$' represents the achievable WC sum rate for the HD setup \cite{JPKR:11}. 
%
%In Fig.~\ref{} the worst-case sum rate of the system is evaluated for different levels of noise intensity ($\sigma_{i,k}^2$).
%In Fig.~\ref{} the worst-case sum rate of the system is evaluated for different levels of communication channel strength ($\Delta_H$)
%In Fig.~\ref{} the worst-case sum rate of the system is evaluated for different levels of transceiver accuracy $\kappa$
%In Fig.~\ref{} the worst-case sum rate of the system is evaluated for different levels of available transmit power $P_i$
%In Fig.~\ref{} the worst-case sum rate of the system is evaluated for different levels of transmit/receiver antennas
%In Fig.~\ref{} the worst-case sum rate of the system is evaluated for different levels of CSI error region radius $\zeta$
%
%
%
%\subsection{Computational complexity} \label{sim_numericalcomplexityanalysis}
%
%In Fig.~\ref{convergence}, an average convergence behavior of the proposed iterative design is observed. 
%
%In Table.~\ref{complexity_time}, the average consumed time of the proposed design process is observed.  

%
%In Fig.~\ref{fig:convergence} - Fig.~\ref{fig:power} the worst-case (WC) achievable sum rate is numerically evaluated. In this respect, 'Scenario~$1$' represents the proposed design in Section~\ref{sec:WMMSE}. 'Scenario~$2$', 'Scenario~$3$', and 'Scenario~$4$' represent a simplified sum-rate maximizing approach, by (respectively) ignoring the impact of distortion signals, i.e., assuming $\kappa=\beta=0$, the impact of CSI inaccuracy, i.e., assuming $\zeta=0$, and jointly ignoring the impacts of chain imperfections and CSI errors. Scenario~$2$ is adopted from the proposed design in \cite{CTLMH:16}, where Scenario~$4$ is previously studied in \cite{Huberman2014, JTLH:12}. Finally, 'Scenario~$5$' represents the achievable WC sum rate for the HD setup \cite{JPKR:11}. 
  %
%In Fig.~\ref{fig:convergence} the average convergence behavior of the proposed iterative method is depicted. As it is observed, the convergence is obtained within 3-10 optimization iterations, which verifies the efficiency of the proposed iterative algorithm in terms of the required computational effort. Moreover, it is observed that such convergence behavior remains relatively constant for different levels of transceiver accuracy.
 %
%In Fig.~\ref{fig:kappa} the obtained guaranteed (worst-case) system sum rate is evaluated for different values of transceiver inaccuracy. It is observed that while the achievable performance in all scenarios degrade as $\kappa=\beta$ increases, the performance of the FD system is more sensitive to the distortion intensity, compared to the HD system, due to the strong self-interference path. The gain of the proposed design ('Scenario~$1$') is particularly observable as the chain inaccuracy increases.  
%
%In Fig.~\ref{fig:zeta} the obtained guaranteed (worst-case) system sum rate is evaluated for different values of channel error intensity. Similar to Fig.~\ref{fig:kappa}, it is observed that the proposed robust design provides a margin of gain as the CSI error radius increases. 
%
%In Fig.~\ref{fig:power} the impact of the maximum transmit power is observed on the achievable (worst-case) system sum rate. It is observed that for a low power system, where the system performance is dominated by the effect of noise, a significant gain is obtained via the proposed FD setup. Nevertheless, the gain obtained by the proposed robust design is marginal. Conversely, in a high power regime where the system performance is dominated by the effect of distortion signals and CSI inaccuracy, the application of a robust design strategy becomes crucial. 
%
%
%Bound gap
%
%convergence 
%
%noise
%kappa and beta
%antenna number
%distance ratio
%zeta
%run time (strategy comparison)
%
%
%\subsection{Tightness of the used lower bound}
%
%\subsection{Sum rate evaluation}
%strategy 1: optimal
%2 : ignore zeta
%3 ignore kappa
%4: ignoring both
%5: jianshu low dynamic range
%6: Jianshu high dynamic range
%7: HD 



%\subsection{Complexity analysis}  \label{sim_numericalcomplexityanalysis}

 

%
%%\begin{table*}[!t] \label{}
  %%\renewcommand{\arraystretch}{1.2}
  %%\caption{Scenarios for SN clusters}\label{tab:Scenarios}
  %%\centering
  %%\begin{tabular}[t]{|l||c|c|c|c|c|}
    %%%\firsthline
		    %%\hline
      %%Scenario &Scenario~$1$ & Scenario~$2$ & Scenario~$3$ & Scenario~$4$ & Scenario~$5$  \\
    %%\hline
    %%& FD setup, proposed design& FD setup, & $|\mathbb{K}| = 16, |\mathbb{L}_k| = 16 $ & $|\mathbb{K}| = 64, |\mathbb{L}_k| = 4 $& $|\mathbb{K}| = 256, |\mathbb{L}_k| =1  $\\
    %%%\lasthline
		    %%\hline
  %%\end{tabular}
%%\end{table*}
%\begin{figure}[!t] 
    %\begin{center}
        %\includegraphics[angle=0,width=\MainFigureSizes]{./Figures/convergence.pdf}
				        %%\fbox{model_rect6.pdf}
    %\caption{{{Average convergence behavior of the proposed iterative method. The proposed method converges to a stable point within 10 optimization iterations. }}} \label{fig:convergence}
    %\end{center} \vspace{-0mm} 
%\end{figure} 
%\begin{figure}[!t] 
    %\begin{center}
        %\includegraphics[angle=0,width=\MainFigureSizes]{./Figures/kappa2.pdf}
				        %%\fbox{model_rect6.pdf}
    %\caption{{{Guaranteed (worst-case) sum rate vs. transceiver inaccuracy ($\kappa = \kappa_i = \beta_j, \; \forall i,j$). Achievable worst case rate as well as the FD system advantage suffers as the transceiver inaccuracy increases.}}} \label{fig:kappa}
    %\end{center} \vspace{-0mm} 
%\end{figure} 
%\begin{figure}[!t] 
    %\begin{center}
        %\includegraphics[angle=0,width=\MainFigureSizes]{./Figures/zeta2.pdf}
				        %%\fbox{model_rect6.pdf}
    %\caption{{{Guaranteed (worst-case) sum rate vs. feasible CSI error radius ($\zeta = \zeta_{ij}, \; \forall i,j$). Achievable rate suffers as the CSI error region expands.}}} \label{fig:zeta}
    %\end{center} \vspace{-0mm} 
%\end{figure} 
%\begin{figure}[!t] 
    %\begin{center}
        %\includegraphics[angle=0,width=\MainFigureSizes]{./Figures/power2.pdf}
				        %%\fbox{model_rect6.pdf}
    %\caption{{{Guaranteed (worst-case) sum rate vs. maximum transmit power ($P = P_{i}, \; \forall i$). Achievable rate is dominated by the effects of CSI error, and transceiver inaccuracy for high power regime. }}} \label{fig:power}
    %\end{center} \vspace{-0mm} 
%\end{figure} 
 %In this section we numerically evaluate the resulting worst-case sum rate of a FD P2P system, using the proposed design. In this respect, we assume that $\ma{H}_{ii}$ follows an uncorrelated Reyligh distribution, with variance $0.01$ for each element and $\ma{H}_{ij} \sim \mathcal{CN}\left( \sqrt{\frac{K_R}{1+K_R}} \ma{H}_0 , \frac{1}{1+K_R} \ma{I}_{N_j} \otimes \ma{I}_{M_i}  \right),\; i\neq j$. $\ma{H}_0$ is matrix with all elements equal to $1$ and $K_R$ is the Rician coefficient. The results are then averaged over 100 channel realizations. Unless otherwise is stated we use the following values to the define our default setup: $N_j = M_i=4$, $K_R =1$, $P_i = 1$~[Watt], $\kappa_i=\beta_j = 0.001$, $\sigma_{\text{n},i}^2=0.1$~[Watt], $\ma{D}_{ij}= \ma{I}$, $\nu_i=1$, $\zeta_{ij} = -15$~[dB], $\forall i,j$. In Fig.~\ref{fig:convergence}-Fig.~\ref{fig:power} the worst-case achievable sum rate is numerically evaluated. In this respect, 'Scenario~$1$' represents the proposed design in Section~\ref{sec:WMMSE}. 'Scenario~$2$', 'Scenario~$3$', and 'Scenario~$4$' represent a simplified sum-rate maximizing approach, by (respectively) ignoring the impact of distortion signals, i.e., assuming $\kappa=\beta=0$, the impact of CSI inaccuracy, i.e., assuming $\zeta=0$, and jontly ignoring the impacts of chain imperfections and CSI errors. Scenario~$2$ is adopted from the proposed design in \cite{CTLMH:16}, where Scenario~$4$ is previously studied in \cite{Huberman2014, JTLH:12}. Finally, 'Scenario~$5$' represents the achievable WC sum rate for the HD setup \cite{JPKR:11}. 
  %
%In Fig.~\ref{fig:convergence} the average convergence behavior of the proposed iterative method is depicted. As it is observed, the convergence is obtained within 10 optimization iterations, which verifies the efficiency of the proposed iterative algorithm in terms of the required computational effort. Moreover, it is observed that such convergence behavior remains relatively constant for different values levels of transceiver accuracy.
 %
%In Fig.~\ref{fig:kappa} the obtained guaranteed (worst-case) system sum rate is evaluated for different values of transceiver inaccuracy. It is observed that while the achievable performance in all scenarios degrade as $\kappa=\beta$ increases, the performance of the FD system is more sensitive to the distortion intensity, compared to the HD system, due to the strong self-interference path. The gain of the proposed design ('Scenario~$1$') is particularly observable as the chain inaccuracy increases. 
%
%In Fig.~\ref{fig:zeta} the obtained guaranteed (worst-case) system sum rate is evaluated for different values of channel error intensity. Similar to Fig.~\ref{fig:kappa}, it is observed that the proposed robust design provides a margin of gain as the CSI error radius increases. 
%
%In Fig.~\ref{fig:power} the impact of the maximum transmit power is observed on the achievable (worst-case) system sum rate. It is ovserved that for the low power system, where the system performance is dominated by the effect of noise, a significant gain is obtained via the proposed FD setup. Conversely, in the high power regime where the system performance is dominated by the effect of distortion signals and CSI inaccuracy, the achievable gain of a FD system is marginal. In all cases, the gain of the proposed design is observable, in comparison to the scenarios with simplifying assumptions.   

==> Sections/sec_abstract.tex <==
 In this paper we address a worst-case weighted sum rate maximization problem for a full-duplex (FD) and multi-carrier point-to-point (P2P) system. The effects of channel-state information (CSI) error, as well as the signal distortion due to hardware impairments are jointly taken into account. This also includes the inter-carrier destruction due to the non-linear distortions in a FD transceiver. Due to the non-tractable structure of the resulting problem, a weighted minimum mean squared error (WMMSE) method is applied to cast the rate maximization problem into a separately convex optimization problem, which can be iteratively solved with a guaranteed convergence to a local optimum. Moreover, a methodology to obtain the least favorable error matrices is proposed by casting the resulting non-convex quadratic optimization into a convex optimization problem. The achievable guaranteed (worst-case) rate is then numerically studied, over different levels of CSI error and transceiver accuracy.


==> Sections/sec_extensions.tex <==

In Section~\ref{sec:WMMSE} we have provided a robust rate maximization framework for a FD-P2P system, which benefits from spatial, and frequency diversity, i.e., a MIMO-MC system. On the other hand, the same framework can be extended to support further algorithm or system concepts which may become relevant in a wider range of applications. In the following we discuss some of the useful extensions which can be implemented with a minimal effort.
   
\subsection{Robust MMSE Transceiver Design} \label{subsec_MMSE}
The optimization in (\ref{eq:global_opt_problem_4}) provides a design for maximizing the system sum rate, where the rate functions are re-structured using the WMMSE method. Alternatively, an optimization problem for obtaining the optimal MMSE system operation can be formulated as
%\begin{subequations} 
\begin{align}  
\underset{{\mathbb{V}}, {\mathbb{U}}}{ \text{min}} \;\; \underset{{\mathbbl{\Delta}}}{\text{max}}  \;\; &\;\; \sum_{i \in \mathbb{I}} \mu_i \sum_{k \in \mathbb{K}} \text{tr} \left( \ma{E}_i^k\right) ,\;\; {\rm s.t.} \;\; \text{(\ref{eq:global_opt_problem_1_power_contraint}),~(\ref{eq:global_opt_problem_1_normbounded_contraint})} \label{eq:global_opt_problem_2_constraints}, \label{MMSE_global_opt_problem}
\end{align} 
%\end{subequations}
where the maximization over ${\mathbbl{\Delta}}$ represents the worst-case channel estimation error in the MMSE sense, and $\mu_i \in \real$ represents the significance of the estimation MSE at communication direction $i$. As it can be observed from (\ref{eq:global_opt_problem_3}), the defined MMSE optimization (\ref{MMSE_global_opt_problem}) can be interpreted as the special case of (\ref{eq:global_opt_problem_3}) by choosing $\nu_i = \mu_i$, and setting $\ma{W}_i^k = \ma{I}_{d_i}$ in the objective and in the definitions of $\ma{c}_{ij}^k$ and $\ma{C}_{ij}^k, \forall i,j \in \mathcal{D}, k \in \mathbb{K}$. As a result, a similar iterative optimization can be employed where at each step a convex sub-problem is solved over ${\mathbb{U}}$ and ${\mathbb{V}}$. Note that unlike the rate maximization case, where the max-min inequality is employed to construct a lower bound of the rate function, the provided framework acts on the exact sum-MSE value as the objective. Moreover, the utilization of the MAX-DET algorithm is not necessary and all sub-problems are presented as a standard SDP, due to the elimination of ${\mathbb{W}}$ from the optimization variables set. 

\subsection{Extended Power Constraints}
System power constraints usually reflect the limitations of battery, or device energy storage. Nevertheless, multiple considerations of power may become relevant for the systems with distributed antennas \cite{5963593}\footnote{In a distributed antenna system a centralized core performs joint transmit/receive processing tasks for all chains. Nevertheless, each antenna unit, or each sub-set of antennas, can be connected to a separate power sources.} or for the transceivers where an accurate operation of the chain elements are crucial. In this respect, a FD transceiver, in particular is sensitive to the operational accuracy of the hardware elements, which may become saturated or inaccurate outside of a given functional range. In this respect the consideration of per transmit antenna power constraint \cite{CZHH:14,7478064}, total or per receive antenna self-interference power constraint as may become relevant \cite{HL:14, Huberman2014, JTLH:12}. 

In order to incorporate this, we generalize the defined power constraint in (\ref{p4_power}) as
\begin{subequations}
\begin{align}  
& \ma{s}_{\text{tx},l}^T \left\lceil \text{diag}\left( \sum_{k \in \mathbb{K} }  \tilde{\ma{V}}_{i}^k \right) \right\rceil_{i \in \mathbb{I} } \leq p_{\text{tx},l},\; l \in \mathbb{C}_{\text{tx}}, \\
&\ma{s}_{\text{rx},l}^T \left\lceil \text{diag}\left( \sum_{k \in \mathbb{K} } \ma{H}_{ij} \tilde{\ma{V}}_{j}^k \ma{H}_{ij}^H \right) \right\rceil_{i \in \mathbb{I}} \leq p_{\text{rx},l}, \; \forall i \neq j \in \mathbb{I},\; l \in \mathbb{C}_{\text{rx}}, \\ 
& \left[\begin{array}{cc} \tilde{\ma{V}}_{i}^k & {{\ma{V}}_{i}^k} \\ {{\ma{V}}_{i}^k}^H & \ma{I}_{d_i}    \end{array} \right] \succeq 0, \; \forall i \in \mathbb{I}, \; k \in \mathbb{K},
\end{align}     
\end{subequations}
where $\tilde{\ma{V}}_{i}^k$ is the transmit covariance in the direction $i$ and subcarrier $k$, and $\ma{s}_{\text{tx},l}$ ($\ma{s}_{\text{rx},l}$) is a selection vector with zero and one elements, and $\mathbb{C}_{\text{tx}}$ ($\mathbb{C}_{\text{rx}}$) are the set of transmit (receive) power constraints\footnote{As an example, the choice $\ma{s}_{\text{tx},l} = [ 1 \ldots 1 ] $ represents a total transmit power from all antennas.}.   

%\subsection{Power Minimization Approach}
%In many applications it is favorable to satisfy a required quality of service, rather than to maximize the system performance. Such consideration results in the minimal resource expenditure, without compromising the required service quality by the user. In order to satisfy a required information rate for the communication direction $i$, namely $I_{\text{req,i}}$, we follow the penalty approach, see \cite[Subsection~3.1.1]{bertsekas1999nonlinear}, by introducing a price term in the objective proportional to the rate deficiency 
%\begin{subequations} \label{eq:sumpower_minimization}
%\begin{align}
%\underset{\mathbb{V}, \mathbb{U}}{ \text{max}} \;\; \underset{\mathbbl{\Delta} }{ \text{min}} \;\; &  \sum_{i \in \mathbb{I}} P_i  + \eta_i \left ( -I_{\text{req},i} + \sum_{k\in \mathbb{K} }  I_i^k \right)  \\
%{\rm s.t.} \;\;     & \text{(\ref{eq:global_opt_problem_1_power_contraint}),~(\ref{eq:global_opt_problem_1_normbounded_contraint})} \label{eq:global_opt_problem_2_constraints},
%\end{align}
%\end{subequations}
%where $\eta_i \in \real$ is the penalty weight and will be adjusted to enforce the satisfaction of the rate constraint. Following the same procedure as in (\ref{eq:model_optimization})-(\ref{eq:global_opt_problem_4}) we restructure the power minimization problem (\ref{eq:sumpower_minimization}) as 
%\begin{subequations}  \label{eq:global_opt_problem_reformulated_sumpowermin}
%\begin{align}
%\underset{\mathbb{V}, \mathbb{U}, \mathbb{W}, \mathcal{T}, \mathcal{C}} {\text{max}} \;\;\; & \sum_{i \in \mathbb{I}} P_i + \eta_i   \bigg(-I_{\text{req},i} + \sum_{k \in \mathbb{K}} 2\text{log} \left|\ma{W}_i^k\right|  + d_i - \sum_{j \in \mathbb{I}} \tau_{ij}^k \bigg) \\
%{\rm s.t.} \;\;     & \ma{\Lambda}_{i,j}^k \succeq 0,  \;\; \forall i,j \in \mathbb{I}, k \in \mathbb{K}, \label{p4_lambda_tau}\\
%&  \ma{\Omega}_i \succeq 0 , \;\;  \forall i \in \mathbb{I}, \label{p4_power}
%\end{align} 
%\end{subequations}
%where the optimization over $\mathbb{V}, \mathbb{U}, \mathbb{W}$ are performed iteratively, similar to that of (\ref{eq:global_opt_problem_4}), where a convex sub-problem for each case. Moreover, the value of $\eta_i$ is updated in the direction of the subgradient $ -I_{\text{req},i} + \sum_{k\in \mathbb{K}}  I_i^k$ after each optimization iteration. Nevertheless, the convergence of the defined algorithm is not necessarily obtained since the satisfaction of the rate constraints may not be feasible for a high value of the rate demand in both communication direction, if the transceiver accuracy is not sufficiently high.        
  
\subsection{Extension to the Multi-User Interference Channel Setup}
The proposed optimization framework in (\ref{}) consideres a multi-carrier FD communication in a P2P setup. Nevertheless, the proposed formulation can be easily extended to a scenario with multiple simultaneously active communication pairs, i.e., a FD interference channel. Such a setup gains high practical relevance, considering the trend of wireless systems towards frequency reuse and network densification, which results in the coexistence of multiple wireless communication links on the same area. In particular, while the proposed design simultaneously accounts for the inherent inaccuracies of a FD system regarding inaccurate CSI and the impacts of hardware impairments, it benefits the performance of an interference channel by simultaneously taking advantage of the additional design freedom. This includes the application of possible duplexing modes\footnote{This is since each communicating pair may now operate as a HD link in two directions, or to act as a FD link where both directions are active.}, as well as spatial (due to multiple antenna setup), and multi-carrier diversities. The two latter cases are in particular beneficial in controlling the additional interference terms in a dense communication setup, by properly assigning different beams/subchannels to the coexisting communication links. 

%In this part we extend the proposed optimization framework for a multi-carrier FD P2P setup, to serve for a more general system with multiple active FD nodes, communicating to a centralized node, i.e., a star topology. This setup in particular presents a multi-user FD cellular topology in the related literature, where all nodes may operate in FD mode, see Subsection~\ref{intro_MUMIMO} for detailed discussion of the related studies. In particular, the proposed approach, while simultaneously accounting for the inherent inaccuracies of a FD system regarding inaccurate CSI and the impacts of hardware impairments, benefits the design of a cellular system by taking advantage of the additional duplexing mode\footenote{This is since each individual link may now operate as a HD link in UL or DL directions, or to act as a FD link where both UL and DL directions are active.}, multi-user, spatial (due to multiple antenna setup), and multi-carrier diversities. The aforementioned factors are particularly effective in combating the usual challenge of FD cellular systems, regarding the co-channel interference (CCI), where the first three factors are most effective in controlling the impacts of the residual self-interference. 
%
In order to extend our design framework, we generalize the definition of the set $\mathbb{I}$ to include all communication links. In this way, each pair includes two communication links which are operating at the opposite directions. Similar to Section~\ref{sec:model}, the channel $\ma{H}_{ii}$ represents the desired channel for the link $i$, where $\ma{H}_{ij}, i \neq j$, represents the interference channel from link $j$ to link $i$. As a result, a similar signal definition is obtained via (\ref{model:transmitsignal}), (\ref{model:rx_signal}), and (\ref{model:ri_estimatedsignal}) where the aggregate interference-plus-noise on the link $i$, and in the subcarrier $k$ is redefined as 
\begin{align}
{\boldsymbol{\nu}}_{i}^k  =\ma{n}_{i}^k +  \ma{e}_{\text{r},i}^k + \ma{\Delta}_{i\bar{i}}^k \ma{V}_{\bar{i}}^k \ma{s}_{\bar{i}}^k + \hspace{-3mm} {\sum_{j \in \{\mathbb{I}\setminus \{i,\bar{i}\}\}}} \hspace{-3mm} \ma{H}_{ij}^k  \ma{x}_{j}^k  +  \hspace{-1mm} \sum_{ j\in \{i,\bar{i}\} } \hspace{-1mm} \ma{H}_{ij}^k \ma{e}_{\text{t},j}^k ,
\end{align}
where $\bar{i}\in\mathbb{I}$ is the index of the communication link at the opposite direction of the link $i$, but among the same pair of nodes. Consequently, the aggregate interference-plus-noise covariance is obtained as (\ref{eq_extension_multiplelinks_aggregate_interference_covariance}). Moreover, following the same procedure as in (\ref{MSE_Matrix})-(\ref{eq:global_opt_problem_4}), a similar optimization structure is obtained where $\ma{c}_{ij}^k$ and $\ma{C}_{ij}^k$ are redefined with the consideration of the new interference terms, see Appendix. 
\begin{figure*}[!hb]
\normalsize
\begin{align} \label{eq_extension_multiplelinks_aggregate_interference_covariance}
\ma{\Sigma}_{i}^k  & = \ma{\Delta}_{i\bar{i}}^k \ma{V}_{\bar{i}}^k{\ma{V}_{\bar{i}}^k}^H {\ma{\Delta}_{i{\bar{i}}}^k}^H +
% \sum_{j \in \mathbb{I}} \ma{\Delta}_{ij}^k \ma{V}_j^k{\ma{V}_j^k}^H {\ma{\Delta}_{ij}^k}^H 
\nonumber \\ & {\sum_{j \in \mathbb{I} }}  \ma{H}_{ij}^k \ma{\Theta}_{\text{tx},j} \text{diag} \left( \sum_{k \in \mathbb{K} } \ma{V}_j^k{\ma{V}_j^k}^H \right)  {\ma{H}_{ij}^k}^H  
+ \ma{\Theta}_{\text{rx},i}  \text{diag} \left( \sum_{k\in\mathbb{K}}  \left( \sigma_{i,k}^2 \ma{I}_{M_i} + {\sum_{j \in \mathbb{I}}}  \ma{H}_{ij}^k  \ma{V}_j^k{\ma{V}_j^k}^H {\ma{H}_{ij}^k}^H \right)    \right)  \nonumber \\ & \;\;\;\; + {\sum_{j \in \{\mathbb{I}\setminus \{i,\bar{i}\}\}}} \ma{H}_{ij}^k  \ma{V}_j^k{\ma{V}_j^k}^H   {\ma{H}_{ij}^k}^H  + \sigma_{i,k}^2 \ma{I}_{M_i}.
\end{align}
\hrulefill
\vspace*{-0mm}
\end{figure*}


%define the set \mathbb{N} representing the communication nodes. Moreover, the set $\mathbb{I}$ is extended to include all active communication links. In this regard, the link $l_i, \; i \in \mathbb{I}$ corresponds to a pair $(n_i,m_i),\; n_i \neq m_i\in \mathbb{N}$ where $n_i$ is the source and $m_i$ is the destination of the communication link $i$. The signal flow in the communication link $i\in\mathbb{I}$ is defined similar to  




==> Sections/sec_into.tex <==
  The main contributions of this paper are as following: 
	\begin{itemize}
	\item In Section\ref{sec:model}, the MC operation of a FD transceiver model is modeled, taking into accounr linear inaccuracies, i.e., CSI error, as well as the non-liner distortion effects. In particular, the existing FD transceiver models are expanded to incorporate a MC setup. Moreover, the behaviour of the recent self-interference cancellation techniques, depending on signal injection methods, are taking into account.   
	\end{itemize}
	
	%\IEEEPARstart{F}{ULL-DUPLEX} transceiver is known with the capability to transmit and receive at the same time and frequency, and hence has the potential to enhance the spectral efficiency~\cite{HBCJMKL:14}. Nevertheless, such systems suffer from the inherent self-interference. Recently, specialized cancellation techniques \cite{Bharadia:14,YLMAC:11,BMK:13,khandani2013two} have demonstrated an adequate level of isolation between Tx and Rx directions to facilitate a FD communication and motivated a wide range of related studies, see, e.g., \cite{HBCJMKL:14,SSDBRW:14}. Nevertheless, such methods are far from perfect in a realistic environment due to i) aging and inherent inaccuracy of the hardware (analog) components, e.g., ADC and digital-to-analog-convertor (DAC) noise, power amplifier and oscillator phase noise in analog domain, as well as ii) inaccurate estimation of the interference paths due to the limited channel coherence time, noise, and limited processing power in digital domain. It is hence essential to take the aforementioned inaccuracies into account for a reliable implementation. 
	%In this regard, a widely used model for the operation of a multiple-antenna FD transceiver is proposed in \cite{}, where a gradient-projection method is proposed for sum rate maximization in a FD P2P setup. A simpler model is then proposed in \cite{}, with the goal of reducing the design complexity by providing a convex optimization design framework. This is done by considering a self-interference power price/threshold that can be successfully tolerated via the available cancellation techniques, and otherwise assuming a perfect (error-free) transceiver operation. Nevrtheless, the application of a simplified model compromises the system performance in the presence of the aforementioned transceiver inaccuracies. Consequently, the consideration of CSI inaccuracy in a FD P2P system is addressed in \cite{} by maximizing the system sum rate, and in \cite{} by minimizing the sum mean-squared-error (MSE). The aforementioned works focus on optimizing the average system performance, where the first and second order statistics of the CSI error is known. Nevertheless, such studied does not provide a guarantee for the provided instantaneous performance, i.e., they only consider the average and not the worst-case system performance under CSI uncertainty. \footnote{The consideration of the average performance maximization is suitable in a fast-fading channel environment, where the CSI, as well as the CSI error changes rapidly. Nevertheless, the worst-case performance maximization is highly relevant for the slow-fading scenarios, since an occasional low quality of the link persists for a relatively longer period of time, see \cite{}.}
	%
%In this work, present a weighted sum rate maximization for a FD and P2P system, following a deterministic representation of the CSI error. In this model the channel matrices are not accurately known, but they are located within a known feasible region with a sufficiently high probability. In the first step, an equivalent WMMSE formulation of the rate maximization problem is presented. Due to the intractable problem structure, a lower bound of the communication rate is formulated, and the resulting problem is structured as a separately convex problem, which results in an iterative convergence to a local optimum point. The impact of the Due to the non-convex   Unlike the statistical approach towards CSI uncertainty, which is suitable for maximizing the average performance, the deterministic approach enables the worst case performance maximization, in the sence that holds over the known feasible channel error region. 
%
%In this work we address the weughted sum rate maximization problem for a FD P2P system, following the comprehensive FD tranceiver model in \cite{}. In the first step, an equivalent WMMSE problem is formulated to instruct the rate maximization problem in a mathematically tractable form. Due to the non convex nature of the worst-case rate function in     
	 %
%
 %
%
%
%\subsection{Mathematical Notation:}
%Throughout this paper, column vectors and matrices are denoted as lower-case and {upper-case} bold letters, respectively. The rank of a matrix, {expectation, trace}, determinant, transpose, conjugate {and} Hermitian transpose are denoted by ${\text{rank} }(\cdot),\; \mathbb{E}(\cdot), \; {\text{ tr}}(\cdot), \;  |\cdot|, \; (\cdot)^{ T},\; (\cdot)^{*}$ {and} $(\cdot)^{ H},$ respectively. The Kronecker product is denoted by $\otimes$. The identity matrix with dimension $K$ is denoted as ${\ma I}_K$ and ${\rm vec}(\cdot)$ operator stacks the elements of a matrix into a vector. {Moreover,} $(\cdot)^{-1}$ represents the inverse of a matrix and $||\cdot||_{2},||\cdot||_{\text{F}}$ {respectively represent the Euclidean and Frobenius norms}. $\left\lfloor \mathbf{A}_i \right \rfloor_{i=1,\ldots,K}$ ($\left\lceil \mathbf{A}_i \right \rceil_{i=1,\ldots,K}$) denotes a tall (fat) matrix, obtained by stacking the matrices $\mathbf{A}_i,~i=1,\ldots, K$. {The set of all positive semi-definite matrices with Hermitian symmetry is denoted by $\mathcal{H}$.}

==> macros.tex <==
\usepackage{bm}
%=== symbols =====================================================
%\newcommand{\ma}[1]{\bm{ #1 }}         % matrix/vector
\newcommand{\ma}[1]{\mathbf{ #1 }}         % matrix/vector

\newcommand{\ten}[1]{\ma{\mathcal #1}} % tensor
\newcommand{\set}[1]{{\mathcal #1}}    % set

\newcommand{\compl}{\mathbb{C}}        % complex-valued numbers
\newcommand{\real}{\mathbb{R}}         % real-valued numbers

\newcommand{\eqdef}{\stackrel{.}{=}} % definition


%=== functional operators ======================================
\newcommand{\realof}[1]{{\rm Re}\left\{ #1 \right\}}           % real part
\newcommand{\imagof}[1]{{\rm Im}\left\{ #1 \right\}}           % imaginary part
\newcommand{\vecof}[1]{{\rm vec}\left\{ #1 \right\}}           % vec operator
\newcommand{\unvecof}[2]{\mathop{\rm unvec}_{#2}\left\{ #1 \right\}}% unvec operator
\newcommand{\diagof}[1]{{\rm diag}\left\{ #1 \right\}}         % diag operator
\newcommand{\traceof}[1]{{\rm tr}\left\{ #1 \right\}}          % trace operator
\newcommand{\twonorm}[1]{\left\|#1\right\|_2}                  % two-norm
\newcommand{\fronorm}[1]{\left\|#1\right\|_{\rm F}}            % Frobenius norm
\newcommand{\honorm}[1]{\left\|#1\right\|_{\rm H}}             % higher-order norm
\newcommand{\maxof}[1]{{\rm max} \left\{ #1 \right\}}          % max
\newcommand{\minof}[1]{{\rm min} \left\{ #1 \right\}}          % min
\newcommand{\expvof}[1]{\mathbb{E}\left\{ #1 \right\}}         % expected value
\newcommand{\expof}[1]{{\rm e}^{#1}}                           % e^{}


%=== other operators ===========================================
\newcommand{\argmax}{\mathop{{\arg \max}}}         % argmax

%=== binary operators ===========================================
\newcommand{\krp}{\diamond}  % Khatri-Rao product: A \krp B
\newcommand{\kron}{\otimes}  % Kronecker product: A \kron B



%=== superscripts ================================================
\newcommand{\degrees}{\circ}   % e.g., 90^\degrees
\newcommand{\trans}{{\rm T}}   % transpose: ^\trans
\newcommand{\herm}{{\rm H}}    % hermitian: ^\herm
\newcommand{\mtrans}{-{\rm T}} % inv.transpose: ^\mtrans
\newcommand{\mherm}{-{\rm H}}  % inv.hermitian: ^\mherm
\newcommand{\pinv}{+}          % pseudo-inverse: ^\pinv
\newcommand{\conj}{*}          % complex conjugate: ^\conj



%=== Tensor stuff ================================================
\newcommand{\tconcat}{\mbox{\Huge \textvisiblespace \hspace{-0.2ex}} \;}
\newcommand{\unf}[2]{\left[ \ten{#1} \right]_{(#2)}}
\newcommand{\unfnot}[2]{\left[ #1 \right]_{(#2)}}


%=== short-hand for colors =======================================
\usepackage{color}
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}

%=== short hand for TWR quantities ===============================
\newcommand{\UT}[1]{\textsf{UT$_#1$}}
\newcommand{\UTM}[2]{\textsf{UT$_#1^{(#2)}$}}
\newcommand{\RS}{{\textsf{RS}}}
\newcommand{\RSf}{\textsf{R}}
\newcommand{\MR}{M_{\rm R}}
\newcommand{\NR}{N_{\rm R}}
\newcommand{\NP}{N_{\rm P}}
\newcommand{\NPi}[1]{N_{\rm P,#1}}
\newcommand{\PT}[1]{P_{{\rm T},#1}}
\newcommand{\PN}[1]{P_{{\rm N},#1}}
\newcommand{\PTR}{P_{{\rm T,R}}}
\newcommand{\PNR}{P_{{\rm N,R}}}
\newcommand{\PTx}{P_{{\rm T}}}
\newcommand{\PNx}{P_{{\rm N}}}

\newcommand{\eff}{{\rm (e)}}
\newcommand{\effT}{{\rm (e)^\trans}}
\newcommand{\effS}{{\rm (e)^2}}
\newcommand{\eq}{{\rm (eq)}}

\newcommand{\target}{{\rm (T)}}

\newcommand{\forw}{{\rm (f)}}
\newcommand{\forwT}{{\rm (f)^\trans}}
\newcommand{\forwH}{{\rm (f)^\herm}}
\newcommand{\backw}{{\rm (b)}}
\newcommand{\backwT}{{\rm (b)^\trans}}
\newcommand{\backwH}{{\rm (b)^\herm}}

\newcommand{\forwn}{{\rm (f,0)}}
\newcommand{\backwn}{{\rm (b,0)}}


%=== pseudo code =================================================
%\newcommand{\algorithmicinitiate}{\textbf{Initiate:}}

%=== other stuff =================================================
\newcommand{\note}[1]{\red{\bfseries #1}}
\newcommand{\TODO}[1]{\par\red{\bfseries ***TODO: #1***}\\}

